Linear Response Theory: A Modern Analytic-Algebraic Approach

Linear response theory is a tool with which one can study systems that are driven out of equilibrium by external perturbations. This monograph presents a thoroughly modern framework to make linear response theory rigorous for a wide array of systems, that is suitable for novel applications such as periodic and random light conductors not yet covered in the literature. Our analytic-algebraic approach, based on von Neumann algebras and associated non-commutative $L^p$-spaces, can deal with discrete and continuous models alike, and include effects of disorder. First, we explain the mathematical setting, give a complete list of our hypotheses and state the main results, which include Kubo and Kubo-Streda formulas. To make our book accessible to a wide audience, we spend Chapters 3 and 4 explaining the mathematical underpinnings such as non-commutative $L^p$- and Sobolev spaces, and generalized commutators. Furthermore, we show how to construct a von Neumann algebras from a topological dynamical system and a 2-cocycle, a procedure which applies to discrete and continuous quantum systems. We dedicate Chapters 5 and 6 to the proofs of our main results. We close the book by sketching a novel application, linear response theory for periodic and random light conductors. This monograph is aimed at advanced students in mathematical physics and researchers.

==> dedication.tex <==
% %
% \begin{dedication}
% 	For Raffa \& Tenko
% \end{dedication}
% %
\dedication{For Raffa \& Tenko}

==> old_stuff.tex <==
%!TEX root = /Users/max/Dropbox/research/Linear response theory/book/linear response theory.tex
\chapter{Proofs (Chapter 6)} % (fold)
\label{cha:proofs_chapter_6}
%
%%% old stuff starting from here %%%
\section{The Kubo formula} % (fold)
\label{Kubo_formula:Kubo_formula}
%
\red{\textbf{Old Stuff: starting from here!!}}

% \subsection{Initial equilibrium states} % (fold)
% \label{Kubo_formula:Kubo_formula:equilibrium_states}
% %
% %
% \begin{lemma}\label{Kubo_formula:lem:Lp_regularity_states}
% 	Let $\rho$ be an initial equilibrium state which verifies $(IS1')$ and $(IS2')$ and $H \in \affil(\Alg)$. Then, under the conditions of Proposition~\ref{dynamics:prop:existence_perturbed_dynamics} it holds that:
% 	%
% 	\begin{enumerate}
% 		\item $J_k \in \affil(\Alg)$ and $J_k \, \rho \in \mathfrak{L}^p(\Alg)$ for all $k = 1 , \ldots , d$, where $J_k$ is the closure of the commutator $\ii [H , X_k]$ initially defined on $\domain_{\mathrm{c}}(H)$.
% 		\item $H \, \eta^{X_k}_t(\rho) \in \mathfrak{L}^p(\Alg)$ for all $t \in \R$.
% 		\item The condition (IS3) is also verified and we have
% 		%
% 		\begin{align*}
% 			H \, \partial_{X_j}(\rho) = - J_k \, \rho + \partial_{X_j}(H \, \rho)
% 			.
% 		\end{align*}
% 		%
% 	\end{enumerate}
% 	%
% \end{lemma}
% %
% %
% \begin{remark}\label{Kubo_formula:remark:Lp_regularity_dropped_nonnegativity}
% 	A closer inspection of the proof below reveals that we do not use the non-negativity of $\rho$, and the Lemma holds if we drop the assumption $\rho \geq 0$.
% \end{remark}
% %
% %
% \begin{proof}
% 	%
% 	\begin{enumerate}
% 		\item Under the hypothesis (TA1), (TA2) and (TA3) one can prove that
% 		%
% 		\begin{align*}
% 			Y_k(t) := \frac{\e^{+ \ii t X_k} \, H \, \e^{- \ii t X_k} - H}{t}
% 		\end{align*}
% 		%
% 		is an element of $\affil(\Alg)$ for all $t \in \R$. This follows since $Y_k(t)$ is the (strong) difference of two elements in $\affil(\Alg)$ which are initially defined and and closable on the dense domain $\domain_{\mathrm{c}}(H)$. Moreover, in view of (TA4) we can define
% 		%
% 		\begin{align*}
% 			Y_k(t) \, \frac{1}{H - \xi} \in \Alg
% 			,
% 			&&
% 			\forall t \in \R
% 			.
% 		\end{align*}
% 		%
% 		Here the crucial argument is that $Y_k(t)$ can be developed a a sum of commutator over $\domain_{\mathrm{c}}(H)$ in view of the {Baker-Campbell-Hausdorff formula} and these commutators are $H$-bounded according to (TA3). This in particular implies $\domain(H) \subseteq \domain \bigl ( Y_k(t) \bigr )$ for all $t \in \R$. Moreover, one can check that
% 		%
% 		\begin{align*}
% 			\slim_{t \to 0} Y_k(t) \, \frac{1}{H - \xi} = J_k \, \frac{1}{H - \xi}
% 		\end{align*}
% 		%
% 		and since $\Alg$ is closed in the SOT one concludes that $J_k \, \frac{1}{H - \xi} \in \Alg$ and $J_k \in \affil(\Alg)$ (see Remark~\ref{framework:remark:algebraic_operations}). Finally, in view of Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}~(2) one concludes that
% 		%
% 		\begin{align}
% 			 \left ( J_k \, \frac{1}{H - \xi} \right ) \, (H - \xi) \, \rho = J_k \, \rho
% 			\label{Kubo_formula:eqn:J_k_rho_insert_resolvent}
% 		\end{align}
% 		%
% 		as elements of $\mathfrak{L}^p(\Alg)$.
% 		\item Just notice that the condition $H \, \rho \in \mathfrak{L}^p(\Alg)$ implies that the domain
% 		%
% 		\begin{align*}
% 			\domain' := \bigl \{
% 			\psi \in \Hil \; \; \vert \; \; \rho \psi \in \domain
% 			(H) \bigr \} \subseteq \Hil
% 		\end{align*}
% 		%
% 		is $\mathcal{T}$-dense and the equality \eqref{Kubo_formula:eqn:J_k_rho_insert_resolvent} is evidently true on $\domain'$. Let $\eta^{X_k}_t$ be $\R$-flow introduced in Section~\ref{framework:nc_Lp_Sobolev_spaces:Sobolev_spaces}. Notice that the equality
% 		%
% 		\begin{align*}
% 			\eta^{X_k}_t(H \, \rho) = \left ( \e^{+ \ii t X_k} \, H \, \e^{- \ii t X_k} \right ) \eta^{X_k}_t(\rho)
% 		\end{align*}
% 		%
% 		holds on the domain $\e^{+ \ii t X_k}[\domain']$ which is still $\mathcal{T}$-dense. Consequently it holds in $\mathfrak{L}^p(\Alg)$ as a consequence of \cite[Proposition 12]{Terp:noncommutative_Lp_spaces:1981}. Moreover, the same argument also implies the equality
% 		%
% 		\begin{align*}
% 			\eta^{X_k}_t(\rho) = \frac{1}{\e^{+ \ii t X_k} \, H \, \e^{- \ii t X_k} - \xi} \; \eta^{X_k}_t \bigl ( (H - \xi) \, \rho \bigr )
% 		\end{align*}
% 		%
% 		as element of $\mathfrak{L}^p(\Alg)$. In conclusion one has
% 		%
% 		\begin{align*}
% 			H \, \eta^{X_k}_t(\rho) \in \mathfrak{L}^p(\Alg)
% 		\end{align*}
% 		%
% 		since
% 		%
% 		\begin{align*}
% 			% CHANGED fix this equation
% 			H \, \frac{1}{\e^{+ \ii t X_k} \, H \, \e^{- \ii t X_k} - \xi}
% 			% &= \Phi_{X_k}^t \left ( H \, \frac{1}{H - \xi} \right ) - t \, Y_k(t) \, \Phi_{X_k}^t \left ( \frac{1}{H - \xi} \right )
% 			% \\
% 			&= \Phi_{X_k}^t \left ( H \, \frac{1}{H - \xi} + t \, Y_k(-t) \, \frac{1}{H - \xi} \right )
% 		\end{align*}
% 		%
% 		is an element of $\Alg$. Moreover, Lemma~\ref{framework:lem:strong_convergence_trace_product} can be used to prove that $H \, \eta^{X_k}_t(\rho) \to H \, \rho$ in the topology of $\mathfrak{L}^p(\Alg)$ when $t \to 0$.
% 		\item The equality
% 		%
% 		\begin{align*}
% 			\frac{1}{H - \xi} \; H \; \frac{\eta^{X_k}_t(\rho) - \rho}{t} &= \frac{1}{H - \xi} \, \left ( \frac{H \, \eta^{X_k}_t(\rho) - \eta^{X_k}_t(H \, \rho)}{t} + \frac{\eta^{X_k}_t(H \, \rho) - H \, \rho}{t} \right )
% 			\\
% 			&= \frac{1}{H - \xi} \, \left ( -Y_k(t) \, \phi_{X_j}^{t}(\rho) + \frac{\phi_{X_j}^{t}(H \, \rho) - H \, \rho}{t} \right )
% 		\end{align*}
% 		%
% 		is well-defined in $\mathfrak{L}^p(\Alg)$. Moreover, both sides have limits for $t \to 0$ in the topology of $\mathfrak{L}^p(\Alg)$, and one obtains
% 		%
% 		\begin{align*}
% 			\left ( \frac{1}{H - \xi} \, H \right ) \, \partial_{X_j}(\rho) = \frac{1}{H - \xi} \, \bigl ( -J_k \, \rho + \partial_{X_j}(H \, \rho) \bigr )
% 			.
% 		\end{align*}
% 		%
% 		The multiplication on both sides by $\frac{1}{H - \xi}$ and the use of the distributive property of Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}
% 		conclude the proof.
% 	\end{enumerate}
% 	%
% \end{proof}
% %
% Let us end this section by discussing the typical form of equilibrium states used in physics. First of all, notice that a sufficient condition to construct an equilibrium state is to define $\rho \:= f(H)$ where $f$ is any positive function in $L^{\infty}(\R)$. In this way the equilibrium condition $\alpha_t^0(\rho) = \rho$ and the positivity condition $\rho \in \Alg^+$ are automatically satisfied. The integrability condition (IS1) instead depends on a combination of various ingredients. In fact from \eqref{framework:eqn:definition_trace_via_functional_calculus} one infers that
% %
% \begin{align}
% 	\mathcal{T}(\rho^p) = \int_0^{+\infty} f(\lambda)^p \; \dd \mu^H_{\mathcal{T}}(\lambda)
% 	\label{Kubo_formula:eqn:p_integrability_condition_rho}
% \end{align}
% %
% where $\dd \mu^H_{\mathcal{T}}$ is the spectral measure of $H$ induced by the trace $\mathcal{T}$ according to the formula
% %
% \begin{align*}
% 	\mu^H_{\mathcal{T}}(\CMcal{O}) := \red{\mathcal{T} \bigl ( \chi_{\CMcal{O}}(H) \bigr )}
% 	,
% 	&&
% 	\CMcal{O} \mbox{ Borel set}
% 	.
% \end{align*}
% %
% We notice that if $\mathcal{T}$ is not finite then the measure $\mu^H_{\mathcal{T}}$ is not normalized. It is of a certain relevance the case in which $\dd \mu^H_{\mathcal{T}}(\lambda) = h_{\mathcal{T}}(\lambda) \, \dd \lambda$ is absolutely continuous with respect to the Lebesgue measure $\dd\lambda$. In this case the integrability properties of $\rho$ can be checked in terms of the $L^1$ property of $f^p \, h_{\mathcal{T}}$. A similar discussion holds for the property (IS2) which requires the finiteness of
% %
% \begin{align}
% 	\mathcal{T} \bigl ( \sabs{H \, \rho}^p \bigr ) = \int_0^{+\infty} f(\lambda)^p \, \sabs{\lambda}^p \, \dd \mu^H_{\mathcal{T}}(\lambda)
% 	,
% 	\label{Kubo_formula:eqn:p_integrability_condition_H_rho}
% \end{align}
% %
% and, at least with respect to the continuous part of the measure, this condition is related to a sufficiently fast decay of the function $f$. On the other hand differentiability properties like (IS1') or (IS2') depend on the particular nature of the derivation and, in turn, by the particular nature of the generators $X_1 , \ldots , X_d$.
%
% Typical ansatz in the literature for the initial equilibrium states are
% %
% \begin{enumerate}[leftmargin=*,label=(\roman*)]
% 	\item $\rho := f(H)$ with $f \in S(\R)$ a Schwartz function;
% 	\item $\rho := f(H) \, b(H)$ with $f \in S(\R)$ a Schwartz function and $b \in M(\R)$ a measurable (aka borelian) function.
% \end{enumerate}
% %
% as and under the slightly stronger condition $\domain(H) \subseteq \domain(H \, \rho)$ one has that $\bigl [ f(H) , \rho \bigr ] = 0$ for all $f \in L^{\infty}(\R)$ (\cf \cite[Proposition~5.26]{schmudgen-12}). The last observation show that it is relevant to make some Assumption~about the property of $\rho$.
% % subsection initial_equilibrium_states (end)
%
%
% \subsection{The Cauchy problem for initial states} % (fold)
% \label{Kubo_formula:Kubo_formula:Cauchy}
% %
% Let us consider the perturbed time-evolution generated by the Hamiltonian $H_{\Phi,\eps}(t)$ related to $H$ via \eqref{main_results:eqn:definition_isospectrally_perturbed_hamiltonian} through $G_{\Phi,\eps}(t)$ described in Hypothesis~\ref{hypothesis:perturbation}. Assume that the system starts in an equilibrium state $\rho$ (\cf Definition~\ref{main_results:defn:initial_equilibrium_state}) at the initial time $t=-\infty$. The initial state $\rho$ can be evolved in time according to different dynamics. The first is given by the \emph{interaction} evolution described in Section~\ref{dynamics:perturbed:interaction_picture}, namely
% %
% \begin{align}
% 	\R \ni t \mapsto \rho_{\mathrm{int}}(t) := \gamma^{\Phi,\eps}_t(\rho) = G_{\Phi,\eps}(t) \, \rho \, G_{\Phi,\eps}(t)^*
% 	.
% 	\label{Kubo_formula:eqn:definition_interaction_evolution}
% \end{align}
% %
% If $\rho \in \Alg^+ \cap \mathfrak{L}^p(\Alg)$ the mapping \eqref{Kubo_formula:eqn:definition_interaction_evolution} is continuous and isometric in the topology of $\mathfrak{L}^p(\Alg)$. Moreover, if $\rho = \rho(H)$ one just has that $\rho_{\mathrm{int}}(t) = \rho \bigl ( H_{\Phi,\eps}(t) \bigr )$ by spectral calculus. The second evolution is dictated by the \emph{full} (perturbed) dynamics induced by $H_{\Phi,\eps}(t)$ and is defined as
% %
% \begin{align}
% 	\R \ni t \mapsto \rho_{\mathrm{full}}(t) := \lim_{s \to -\infty} \alpha^{\Phi,\eps}_{(t,s)}(\rho)
% 	\label{Kubo_formula:eqn:definition_full_evolution}
% \end{align}
% %
% where $\alpha^{\Phi,\eps}_{(t,s)}$ is the perturbed evolution in $\mathfrak{L}^p(\Alg)$ introduced in Consequence~\ref{main_results:conseq:perturbed_evolution} and the limit has to be understood in the sense of the topology of $\mathfrak{L}^p(\Alg)$ whenever $\rho \in \Alg^+ \cap \mathfrak{L}^p(\Alg)$. The existence of the limit \eqref{Kubo_formula:eqn:definition_full_evolution} is \emph{a priori} not obvious, and in fact it needs some additional conditions.
% %
% \begin{proposition}\label{Kubo_formula:prop:existence_limit_dynamics}
% 	Let $\rho$ by an initial equilibrium state which verifies (IS1') and (IS2) and $\rho_{\mathrm{int}}(t)$ the {interaction} evolution prescribed by \eqref{Kubo_formula:eqn:definition_interaction_evolution}. Under the validity of hypothesis of Proposition~\ref{dynamics:prop:existence_perturbed_dynamics} the limit \eqref{Kubo_formula:eqn:definition_full_evolution} which defines $\rho_{\mathrm{full}}(t)$ exists and it holds true that
% 	%
% 	\begin{align}
% 		\rho_{\mathrm{full}}(t) = \rho_{\mathrm{int}}(t) - \sum_{j = 1}^d \Phi_j \; \int_{-\infty}^t \dd \tau \; \switch(\tau) f_j(\tau) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )
% 		.
% 		\label{Kubo_formula:eqn:difference_full_interaction_dynamics}
% 	\end{align}
% 	%
% \end{proposition}
% %
% %
% \begin{proof}
% 	Condition (IS2) and Lemma~\ref{dynamics:lem:auxilary_difference_dynamics} ensure that $H_{\Phi,\eps}(s) \, \rho_{\mathrm{int}}(s) \in \mathfrak{L}^p(\Alg)$, hence one can apply Proposition~\ref{dynamics:prop:properties_perturbed_dynamics} (2) to differentiate $\alpha^{\Phi,\eps}_{(t,s)} \bigl (\rho_{\mathrm{int}}(s) \bigr )$. The Leibniz rule leads to
% 	%
% 	\begin{align*}
% 		\frac{\dd}{\dd s} \alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) =
% 		\ii \, \alpha^{\Phi,\eps}_{(t,s)} \left ( \bigl [ H_{\Phi,\eps}(s) \, , \, \rho_{\mathrm{int}}(s)\bigr ]_{\ddagger} \right ) +
% 		\alpha^{\Phi,\eps}_{(t,s)} \Bigl ( \tfrac{\dd}{\dd s}\gamma^{\Phi,\eps}_s(\rho) \Bigr )
% 		.
% 	\end{align*}
% 	%
% 	The generalized commutator is well-defined and form Lemma~\ref{dynamics:eqn:evolution_H_rho} and the equilibrium condition \eqref{main_results:eqn:selfadjointness_product_H_rho} it follows that
% 	%
% 	\begin{align}
% 		\bigl [ H_{\Phi,\eps}(s) \, , \, \rho_{\mathrm{int}}(s) \bigr ]_{\ddagger} = \gamma^{\Phi,\eps}_s \bigl ( H \, \rho - (H \, \rho)^* \bigr ) = 0
% 		.
% 		\label{Kubo_formula:eqn:evaluation_generalized_commutator_H_per_rho_int}
% 	\end{align}
% 	%
% 	Condition (IS1') allows us to apply Proposition~\ref{dynamics:prop:interaction_dynamics}~(3) and one gets
% 	%
% 	\begin{align*}
% 		\frac{\dd}{\dd s} \alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) =
% 		\alpha^{\Phi,\eps}_{(t,s)} \left ( \switch(s)\,\sum_{k = 1}^d \Phi_k \, f_k(s) \, \partial_{X_k} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) \right ) .
% 	\end{align*}
% 	%
% 	An integration provides
% 	%
% 	\begin{align*}
% 		\alpha^{\Phi,\eps}_{(t,t)} \bigl ( \rho_{\mathrm{int}}(t) \bigr ) - \alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) = \sum_{j = 1}^d \Phi_j \; \int_s^t \dd \tau \; \switch(\tau) \, f_j(\tau) \;
% 		\alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )
% 		.
% 	\end{align*}
% 	%
% 	Observe that $\alpha^{\Phi,\eps}_{(t,t)} \bigl ( \rho_{\mathrm{int}}(t) \bigr ) = \rho_{\mathrm{int}}(t)$. Therefore, to obtain the formula \eqref{Kubo_formula:eqn:difference_full_interaction_dynamics} one needs to take the limit $s \to -\infty$ of the last equation. Since
% 	%
% 	\begin{align*}
% 		\Bnorm{\alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )}_p = \bnorm{\partial_{X_j}(\rho)}_p < +\infty
% 	\end{align*}
% 	%
% 	in view of the condition (IS1') and the isometry of the maps $\alpha^{\Phi,\eps}_{(t,\tau)}$ and $\gamma^{\Phi,\eps}_s$, it follows that the convergence of the Bochner integral is guaranteed by the integrability condition \eqref{main_results:eqn:integrability_condition}. This fact proves the existence of the limit $\lim_{s \to -\infty} \alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) $. The equality
% 	%
% 	\begin{align*}
% 		\lim_{s \to -\infty} \alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr )
% 		 = \rho_{\mathrm{full}}(t)
% 		 ,
% 	\end{align*}
% 	%
% 	necessary to conclude the proof of \eqref{Kubo_formula:eqn:difference_full_interaction_dynamics}, follows from
% 	%
% 	\begin{align*}
% 		\Bnorm{\alpha^{\Phi,\eps}_{(t,s)} \bigl ( \rho_{\mathrm{int}}(s) \bigr ) - \alpha^{\Phi,\eps}_{(t,s)}(\rho)}_p = \bnorm{\gamma^{\Phi,\eps}_s(\rho) - \rho}_p
% 	\end{align*}
% 	%
% 	and Proposition~\ref{dynamics:prop:interaction_dynamics}~(1).
% \end{proof}
% %
% The next properties are consequences of the definitions \eqref{Kubo_formula:eqn:definition_interaction_evolution} and \eqref{Kubo_formula:eqn:definition_full_evolution}.
%
%
%
% %
% \begin{remark}
% 	It is worth noting that if one replace Assumption~(IS2) with its stronger version (IS2') in the claim of Theorem~\ref{main_results:thm:comparison_dynamics}, then the condition (IS3) is automatically verified due to Lemma~\ref{Kubo_formula:lem:Lp_regularity_states}~(3).
% \end{remark}
% %
% % subsection the_cauchy_problem_for_initial_states (end)
%
%
% \subsection{Current-type observables} % (fold)
% \label{Kubo_formula:Kubo_formula:current_observables}
% %
% In this section we want to justify Hypothesis~\ref{hypothesis:current} which introduces the notion of current-type observable.
%
% Let us recall that under the the Hypothesis~\ref{hypothesis:current}~(i)–(iii) one can define the \emph{unperturbed} vector-valued \emph{current operator} $\mathbf{J} := (J_1,\ldots ,J_d)$,
% %
% \begin{align*}
% 	J_k := \ii [H , X_k] = - \partial_{X_j}(H)
% \end{align*}
% %
% which is initially defined on the dense set $\domain_{\mathrm{c}}(H)$. If $\mathbf{J}$ represents the current generated by the Hamiltonian $H$ one can similarly define the \emph{instantaneously perturbed} current operator generated by the perturbed Hamiltonian $H_{\Phi,\eps}(t) = G_{\Phi,\eps}(t) \, H \, G_{\Phi,\eps}(t)^*$ by
% %
% \begin{align*}
% 	\mathbf{J}_{\Phi,\eps}(t) := G_{\Phi,\eps}(t) \; \mathbf{J} \; G_{\Phi,\eps}(t)^* = \ii \bigl [ H_{\Phi,\eps}(t) \, , \, \mathbf{X} \bigr ]
% \end{align*}
% %
% where the second equality holds (initially) on the dense domain $\domain_{\mathrm{c}}(H)$ under the conditions Hypothesis~\ref{hypothesis:current}~(i)–(iii). Similarly, we can associate to the \emph{unperturbed} tensor of order $r$
% %
% \begin{align*}
% 	\mathbf{J}^{(r)} := \bigl \{ J_{\kappa} \bigr \}_{\abs{\kappa} = r}
% 	,
% 	&&
% 	1 \leqslant r \leqslant N
% 	,
% \end{align*}
% %
% its \emph{instantaneously} perturbed counterpart,
% %
% \begin{align*}
% 	\mathbf{J}^{(r)}_{\Phi,\eps}(t) := G_{\Phi,\eps}(t) \; \mathbf{J}^{(r)} \, G_{\Phi,\eps}(t)^*
% 	.
% \end{align*}
% %
% Since the current density operators are relevant for applications we study in the next lemma some of their properties.
% %
% \begin{lemma}\label{lemma:propert_current_oper}
% 	Suppose Hypotheses~\ref{hypothesis:trace}–\ref{hypothesis:state} hold true. Then $\mathbf{J}^{(r)}_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \in \mathfrak{L}^p(\Alg)$ for all $t \in \R$ and
% 	%
% 	\begin{align*}
% 		\lim_{t \to -\infty} \mathbf{J}^{(r)}_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) = \mathbf{J}^{(r)} \, \rho
% 	\end{align*}
% 	%
% 	in the topology of $\mathfrak{L}^p(\Alg)$.
% \end{lemma}
% %
% %
% \begin{proof}
% 	Notice that one of the implications of Theorem~\ref{main_results:thm:comparison_dynamics} is that $H_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \in \mathfrak{L}^p(\Alg)$ for all $t \in \R$. Moreover, the equality
% 	%
% 	\begin{align*}
% 		H_{\Phi,\eps}(t) \, &\rho_{\mathrm{full}}(t)
% 		= \\
% 		&
% 		= \gamma^{\Phi,\eps}_t \bigl ( H \, \rho \bigr ) - \sum_{j = 1}^d \Phi_j \; \int_{-\infty}^t \dd \tau \; \rr{sf}_{\eps}(\tau)\; f_j(\tau) \; H_{\Phi,\eps}(t) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )
% 	\end{align*}
% 	%
% 	which follows from Proposition~\ref{Kubo_formula:prop:existence_limit_dynamics} (the existence of the Bochner integral is justified in the proof of Theorem~\ref{main_results:thm:comparison_dynamics}). Lemma~\ref{dynamics:lem:auxilary_difference_dynamics} implies $H_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \to H \, \rho$ when $t \to -\infty$ in the topology of $\mathfrak{L}^p(\Alg)$. On the other hand the equality
% 	%
% 	\begin{align}
% 		\mathbf{J}^{(r)}_{\Phi,\eps}(t) \, \frac{1}{H_{\Phi,\eps}(t) - \xi} &= G_{\Phi,\eps}(t) \; \mathbf{J}^{(r)} \; \frac{1}{H - \xi} \; G_{\Phi,\eps}(t)^*
% 		\notag \\
% 		&= \gamma^{\Phi,\eps}_t \left ( \mathbf{J}^{(r)} \, \frac{1}{H - \xi} \right )
% 		\label{Kubo_formula:eqn:lim_Jtensor_rho}
% 	\end{align}
% 	%
% 	shows that left-hand side is a tensor with components in $\Alg$ for all $t$,
% 	%
% 	\begin{align*}
% 		J_{\kappa} \, \frac{1}{H - \xi} \in \Alg
% 		.
% 	\end{align*}
% 	%
% 	Therefore we can modify the arguments for $r = 1$ in the proof of Lemma~\ref{Kubo_formula:lem:Lp_regularity_states}~(1) and combine it with Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}~(2),
% 	%
% 	\begin{align*}
% 		\mathbf{J}^{(r)}_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) = \left ( \mathbf{J}^{(r)}_{\Phi,\eps}(t) \, \frac{1}{H_{\Phi,\eps}(t) - \xi} \right )
% 		\; \Bigl ( \bigl ( H_{\Phi,\eps}(t) - \xi \bigr ) \, \rho_{\mathrm{full}}(t) \Bigr )
% 		,
% 	\end{align*}
% 	%
% 	to conclude $\mathbf{J}_{\Phi,\eps}^{(r)}(t) \, \rho_{\mathrm{full}}(t) \in \mathfrak{L}^p(\Alg)$.
%
% 	To prove the existence of the limit, we note that the sequence involved in
% 	%
% 	\begin{align*}
% 		\slim_{t \to -\infty} \gamma^{\Phi,\eps}_t \left ( \mathbf{J}^{(r)} \, \frac{1}{H - \xi} \right ) = \mathbf{J}^{(r)} \, \frac{1}{H - \xi}
% 	\end{align*}
% 	%
% 	is equibounded and converging with respect to the SOT. Hence, we can write
% 	%
% 	\begin{align*}
% 		\mathbf{J}^{(r)}_{\Phi,\eps}(t) \, &\rho_{\mathrm{full}}(t) - \mathbf{J}^{(r)} \, \rho
% 		= \\
% 		&= \gamma^{\Phi,\eps}_t \left ( \mathbf{J}^{(r)} \, \frac{1}{H - \xi} \right )
% 		\; \Bigl ( \bigl ( H_{\Phi,\eps}(t) - \xi \bigr ) \, \rho_{\mathrm{full}}(t) - (H - \xi) \, \rho \Bigr )
% 		+ \\
% 		&\qquad
% 		+ \left ( \gamma^{\Phi,\eps}_t \left ( \mathbf{J}^{(r)} \, \frac{1}{H - \xi} \right ) - \mathbf{J}^{(r)} \, \frac{1}{H - \xi} \right ) \, (H - \xi) \, \rho
% 	\end{align*}
% 	%
% 	where both summands on the right-hand side converge to zero as $t \to -\infty$ in the topology of $\mathfrak{L}^p(\Alg)$. This concludes the proof.
% \end{proof}
% %
% A comparison with Hypothesis~\ref{hypothesis:current} shows that the notions of current-type observable is inspired by the results in Lemma~\ref{Kubo_formula:lem:Lp_regularity_states} and Lemma~\ref{lemma:propert_current_oper}.
% % subsection current_type_observables (end)
%
%
% \subsection{The macroscopic net current and conductivity tensor} % (fold)
% \label{Kubo_formula:Kubo_formula:macroscopic_current}
% %
% In the situation described in Definition~\ref{main_results:defn:current} one can introduce the \emph{macroscopic net current}
% %
% \begin{align}
% 	\mathscr{J}^{\Phi,\eps}[J,\rho](t) := \mathcal{T} \bigl ( J_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \bigr ) - \mathcal{T}(J \, \rho)
% 	\label{Kubo_formula:eqn:net_macroscopic_current}
% \end{align}
% %
% associated with the current-type observable $J$. This quantity is a measure of the difference of the net flow of current due to $J$ with respect to the state $\rho$ between the unperturbed and the perturbed dynamics when a perturbation field $\pmb{\Phi}$ is switched on adiabatically at rate $\eps > 0$ between the initial time $-\infty$ and the final time $t$.
% %
% \begin{remark}[Equilibrium conditions]\label{Kubo_formula:remark:equilibrium_conditions_current}
% 	% TODO Rewrite this remark
% 	There are two case in which the system is in equilibrium. The first is when $t \to -\infty$. In fact the continuity condition~(ii) of Definition~\ref{main_results:defn:current} ensures
% 	%
% 	\begin{align*}
% 		\lim_{t \to -\infty} \mathscr{J}^{\Phi,\eps}[J,\rho](t) = \lim_{t \to -\infty} \mathcal{T} \bigl (J_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \bigr ) - \mathcal{T}(J \, \rho) = 0
% 		.
% 	\end{align*}
% 	%
% 	In the particular case of a finite initial time $t_0 > -\infty$ one has also the stronger condition
% 	%
% 	\begin{align*}
% 		\mathscr{J}^{\Phi,\eps}[J,\rho](t) = \mathcal{T} \bigl ( J_{\Phi,\eps}(t_0) \, \rho_{\mathrm{full}}(t_0) \bigr ) - \mathcal{T}(J \, \rho) = 0
% 		&&
% 		\forall t \leqslant t_0
% 	\end{align*}
% 	%
% 	due to $J_{\Phi,\eps}(t) = J_{\Phi,\eps}(t_0) = J$ and $\rho_{\mathrm{full}}(t) = \rho_{\mathrm{full}}(t_0) = \rho$ for all $t \leqslant t_0$. In many situations one expects also a \emph{null net current} at the equilibrium, namely
% 	%
% 	\begin{align}
% 		\lim_{t \to -\infty} \mathcal{T} \bigl ( J_{\Phi,\eps}(t) \, \rho_{\mathrm{full}}(t) \bigr ) = \mathcal{T}(J \, \rho) = 0
% 		.
% 		\label{Kubo_formula:eqn:no_go_equation}
% 	\end{align}
% 	%
% 	Other than Definition~\ref{main_results:defn:current}~(i)–(ii), the validity of condition \eqref{Kubo_formula:eqn:no_go_equation} depends also on a lot of factors like the nature of $H$, the generators $\mathbf{X}$ and the initial state $\rho$.
% 	% CHANGED Very vague, make this sentencxe more precise. > No-go theorem has been removed.
% 	% In some situations \eqref{Kubo_formula:eqn:no_go_equation} can be derived by some structural property of the basic elements of the theory (see Lemma~\ref{Kubo_formula:lem:no_go_theorem} below).
% 	The second equilibrium condition concern the vanishing of the perturbation field $\pmb{\Phi}$. Clearly, in the limit of vanishing perturbation at fixed $\eps > 0$ the net current vanishes,
% 	%
% 	\begin{align*}
% 		\mathscr{J}_{\Phi=0,\eps}[J,\rho](t) = \mathcal{T} \bigl ( J_{\Phi=0,\eps}(t) \, \rho_{\mathrm{full}}(t) \bigr ) - \mathcal{T}(J\rho) = 0
% 		,
% 	\end{align*}
% 	%
% 	since $G_{\Phi=0,\eps}(t) = \id$ implies $J_{\Phi=0,\eps}(t) = J$, $H_{\Phi=0,\eps} = H$ and $\rho_{\mathrm{full}}(t) = \rho$ as $\rho$ is an equilibrium state. The continuity of
% 	%
% 	\begin{align*}
% 		\lim_{\Phi \to 0} \mathscr{J}^{\Phi,\eps}[J,\rho](t) = \mathscr{J}_{\Phi=0,\eps}[J,\rho](t) = 0
% 	\end{align*}
% 	%
% 	% FIXME Really, does it? We have dropped the distinction between
% 	at $\pmb{\Phi} = 0$ requires some additional assumptions and will be studied in Lemma~\ref{Kubo_formula:lem:existence_integral_net_current} below.
% \end{remark}
% %
% % FIXME Rewrite this bit using the original definition of $\mathscr{J}^{\Phi,\eps}[J,\rho](t)$ which involves $\rho_{\mathrm{int}}(t)$ and use expression for $\rho_{\mathrm{full}}(t) - \rho_{\mathrm{int}}(t)$.
% Let us assume that all the condition for the validity of the equation \eqref{Kubo_formula:eqn:difference_full_interaction_dynamics} are verified. In this case one can rewrite (for the moment formally) the density current associated to a current-type observable $J$ as
% %
% \begin{align}
% 	\mathscr{J}^{\Phi,\eps}[J,\rho](t) &= \Delta_{J,\rho}(t)
% 	\, + \notag \\
% 	&\qquad
% 	 - \ii \sum_{j = 1}^d \Phi_j \; \mathcal{T} \left ( J_{\Phi,\eps}(t) \; \int_{-\infty}^t \dd \tau \; \switch(\tau) \, f_j(\tau) \, \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr ) \right )
% 	 \label{Kubo_formula:eqn:splitting_net_current}
% \end{align}
% %
% where
% %
% \begin{align*}
% 	\Delta_{J,\rho}(t) := \mathcal{T}\big(J_{\Phi,\eps}(t) \, \rho_{\mathrm{int}}(t)\big) - \mathcal{T}(J\rho)
% 	.
% \end{align*}
% %
% Notice that the conditions in Definition~\ref{main_results:defn:current} ensure not only that $\Delta_{J,\rho}(t)$ is well-defined but also $\Delta_{J,\rho}(t) = 0$ for all $t \in \R$ due to the equality
% %
% \begin{align*}
% 	J_{\Phi,\eps}(t) \, \rho_{\mathrm{int}}(t) = \gamma^{\Phi,\eps}_t(J \, \rho)
% \end{align*}
% %
% (\cf Lemma~\ref{dynamics:lem:auxilary_difference_dynamics}) and the invariance of the trace under the evolution $\gamma^{\Phi,\eps}_t$. Moreover, point~(iii) of Definition~\ref{main_results:defn:current} ensures that
% %
% \begin{align*}
% 	J_{\Phi,\eps}(t) \, &\alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )
% 	= \\
% 	&= \gamma^{\Phi,\eps}_t \left ( J \, \frac{1}{H - \xi} \right )  \Bigl ( \bigl ( H_{\Phi,\eps}(t) - \xi \bigr ) \, \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr ) \Bigr )
% 	,
% \end{align*}
% %
% and this allows the passage of $J_{\Phi,\eps}(t)$ inside the integration symbol with the same argument used in the proof of the equality~\eqref{Kubo_formula:eqn:linearity_integral_product_Alg_Lp} \textbf{(reference to linearity product $\affil(\Alg)$ and $\mathfrak{L}^p(\Alg)$)}. This allows to rewrite the formula \eqref{Kubo_formula:eqn:splitting_net_current} as
% %
% \begin{align}
% 	\mathscr{J}^{\Phi,\eps}[J,\rho](t) := - \ii \sum_{j = 1}^d \Phi_j \; \mathcal{T} \left ( \int_{-\infty}^t \dd \tau \; \switch(\tau) \; f_j(\tau) \; J_{\Phi,\eps}(t) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr ) \right )
% 	.
% 	\label{Kubo_formula:eqn:macroscopic_current_explicit}
% \end{align}
% %
% The convergence of the integral will be discussed in the following lemma.
% %
% \begin{lemma}\label{Kubo_formula:lem:existence_integral_net_current}
% 	Suppose Hypotheses~\ref{hypothesis:trace}–\ref{hypothesis:current} hold true and the state $\rho$ satisfies Hypothesis~\ref{hypothesis:state} for $p = 1$. Moreover, let $J$ be a current-type observable in the sense of Definition~\ref{main_results:defn:current}. Then the macroscopic net current $\mathscr{J}^{\Phi,\eps}[J,\rho](t)$ defined by \eqref{Kubo_formula:eqn:net_macroscopic_current} is continuous in the perturbation field $\pmb{\Phi}$ and vanishes in the limit
% 	%
% 	\begin{align*}
% 		\lim_{\Phi \to 0} \mathscr{J}^{\Phi,\eps}[J,\rho](t) = \mathscr{J}^{0,\eps}[J,\rho](t)
% 		= 0
% 		&&
% 		\forall t \in \R
% 		.
% 	\end{align*}
% 	%
% \end{lemma}
% %
% %
% \begin{remark}
% 	Note that the differentiability of $H \, \rho$ in $\mathfrak{L}^1(\Alg)$ is not necessary.
% \end{remark}
% %
% %
% \begin{proof}
% 	As for the derivation of the inequality \eqref{Kubo_formula:eqn:bound_generalized_commutator} one has
% 	%
% 	\begin{align}
% 		\norm{J_{\Phi,\eps}(t) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )}_1 &\leqslant K_t \; \norm{J \, \frac{1}{H - \xi}} \; \bnorm{(H - \xi) \, \partial_{X_j}(\rho)}_1
% 		\label{Kubo_formula:eqn:trace_norm_estimate_J_alpha_partial_rho}
% 	\end{align}
% 	%
% 	where $K_t = \max_{\sabs{\Phi} \leqslant 1} K_t^{\Phi}$ and the constant $K_t^\Phi$ is defined in \eqref{dynamics:eqn:sup_s_norm_bound_M_ts}. The existence of such a $K_t$ can be inferred from the discussion in the proof of Proposition~\ref{dynamics:prop:M_limit_Phi}. Inequality \eqref{Kubo_formula:eqn:trace_norm_estimate_J_alpha_partial_rho} ensures that the integral in \eqref{Kubo_formula:eqn:macroscopic_current_explicit} is well-defined in the Bochner sense. Moreover, the manifest linearity in the components of the field which appear in the formula \eqref{Kubo_formula:eqn:macroscopic_current_explicit} in conjunction with the strong continuity of $\alpha^{\Phi,\eps}_{(t,s)}$ with respect to $\pmb{\Phi}$ in $\mathfrak{L}^p(\Alg)$ (Proposition~\ref{dynamics:prop:continuity_perturbed_dynamics_field_strength}) suffice to justify the vanishing of the limit.
% \end{proof}
% %
% %
% \begin{remark}\label{Kubo_formula:remark:trace_norm_estimate_J_alpha_partial_rho}
% 	As a byproduct of the proof of Lemma~\ref{Kubo_formula:lem:existence_integral_net_current} one has that the integral which appears in the formula \eqref{Kubo_formula:eqn:macroscopic_current_explicit} is convergent in the topology of $\mathfrak{L}^1(\Alg)$ as a Bochner integral. The continuity of the trace with respect to the topology of $\mathfrak{L}^1(\Alg)$ and the inequality
% 	%
% 	\begin{align*}
% 		\abs{\mathcal{T} \Bigl ( J_{\Phi,\eps}(t) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr ) \Bigr )}
% 		\leqslant \norm{J_{\Phi,\eps}(t) \; \alpha^{\Phi,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigr ) \bigr )}_1
% 	\end{align*}
% 	%
% 	ensures that one can move the trace $\mathcal{T}$ inside the symbol of integration in equation \eqref{Kubo_formula:eqn:macroscopic_current_explicit}.
% \end{remark}
% %
% For the aims of LRT one needs to go beyond the continuity of $\mathscr{J}^{\Phi,\eps}[J,\rho](t)$ in $\Phi$ and one want to obtain an expansion of the type
% %
% \begin{align*}
% 	\mathscr{J}^{\Phi,\eps}[J,\rho](t) = \sum_{k = 1}^d \Phi_k \, \sigma^{\eps}_k[J,\rho](t) + \order(\Phi^2)
% 	.
% \end{align*}
% %
% where the \emph{conductivity tensor} $\bigl \{ \sigma^{\eps}_k[J,\rho](t) \bigr \}_{1 \leqslant k \leqslant d}$ is given in Definition~\ref{main_results:defn:conductivity_tensor}.
% % subsection the_macroscopic_current_and_conductivity_tensor (end)
% 
% 
% \subsection{The Kubo formula for the conductivity tensor} % (fold)
% \label{Kubo_formula:Kubo_formula:Kubo_formula_conductivity}
% %
% % %
% % \begin{proof}[Proof of Theorem~\ref{main_results:thm:Kubo_formula}]
% % 	% FIXME Add necessary assumptions
% % 	% FIXME The definition implies nothing, it \emph{assumes} the existence of limits
% % 	\red{State the necessary assumptions here.} Definition~\ref{main_results:defn:conductivity_tensor},
% % 	formula \eqref{Kubo_formula:eqn:macroscopic_current_explicit} and Lemma~\ref{Kubo_formula:lem:existence_integral_net_current} imply
% % 	%
% % 	\begin{align*}
% % 		 \sigma^{\eps}_k[J,\rho](t) &= \lim_{\Phi_k \to 0} \frac{\mathscr{J}_{(0,\ldots,\Phi_k,\ldots,0),\eps}[J,\rho](t) - \mathscr{J}^{0,\eps}[J,\rho](t)}{\Phi_k}
% % 		 \\
% % 		 &= - \ii \lim_{\Phi_k\to 0} \mathcal{T} \left ( \int_{-\infty}^t \dd \tau \; \switch(\tau) f_k(\tau) \; J_{\Phi_k,\eps}(t) \; \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \right )
% % 	\end{align*}
% % 	%
% % 	where also $\rho_{\mathrm{int}}(\tau)=\gamma_\tau^{\Phi_k,\eps}(\rho)$
% % 	depends on $\Phi_k$ through the gauge transformation $G_{\Phi_k,\eps}(t)$ (we will use $\Phi_k$ as a short hand for $(0,\ldots,\Phi_k,\ldots,0)$). The inequality \eqref{Kubo_formula:eqn:trace_norm_estimate_J_alpha_partial_rho}, Lemma~\ref{Kubo_formula:lem:existence_integral_net_current} and the Lebesgue's dominated convergence theorem allow to move the limit inside the integral and one obtains
% % 	%
% % 	\begin{align*}
% % 		 \sigma^{\eps}_k[J,\rho](t) &= - \ii \int_{-\infty}^t \dd \tau \; \switch(\tau) \; f_k( \tau) \; \lim_{\Phi_k \to 0} \mathcal{T} \left ( J_{\Phi_k,\eps}(t) \; \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \right )
% % 	\end{align*}
% % 	%
% % 	where we note in passing that the existence of the trace is guaranteed by the fact that it is evaluated on an element in $\mathfrak{L}^1(\Alg)$. After some manipulations one can write
% % 	%
% % 	\begin{align*}
% % 		\mathcal{T} \Bigl ( J_{\Phi_k,\eps}&(t) \; \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \Bigr )
% % 		=
% % 		\\
% % 		&= \mathcal{T} \left (
% % 		\gamma^{\Phi_k,\eps}_t \left ( J \, \frac{1}{H - \xi} \right ) \; \biggl ( \bigl ( H_{\Phi_k,\eps}(t) - \xi \bigr ) \; \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \biggr ) \right )
% % 		\\
% % 		&= \mathcal{T} \left (
% % 		\gamma^{\Phi_k,\eps}_t \left ( J \, \frac{1}{H - \xi} \right ) \; \left ( \bigl ( H_{\Phi_k,\eps}(t) - \xi \bigr ) \; U_{\Phi_k,\eps}(t,\tau) \; \frac{1}{H_{\Phi_k,\eps}(\tau) - \xi} \right ) \;
% % 		\cdot \right . \\
% % 		&\qquad \quad \biggl . \cdot \,
% % 		\gamma^{\Phi_k,\eps}_{\tau} \bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr ) \; U_{\Phi_k,\eps}(\tau,t) \biggr )
% % 		\\
% % 		&= \mathcal{T} \left ( U_{\Phi_k,\eps}(\tau,t) \;
% % 		\gamma^{\Phi_k,\eps}_t \left ( J \; \frac{1}{H - \xi} \right ) \; M_{\Phi_k,\eps}(t,\tau) \; \gamma^{\Phi_k,\eps}_{\tau}\bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr ) \right )
% % 		.
% % 	\end{align*}
% % 	%
% % 	where Lemma~\ref{framework:lem:extension_algebra_unbounded_operators} and the cyclic property of the trace have been used repeatedly. The operator $M_{\Phi_k,\eps}(t,\tau)$ is defined by \eqref{dynamics:eqn:definition_M_ts}. Therefore one gets
% % 	%
% % 	\begin{align*}
% % 		\lim_{\Phi_k \to 0} \mathcal{T} \left ( J_{\Phi_k,\eps}(t) \, \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \right ) =
% % 		\lim_{\Phi_k\to 0} \mathcal{T} \left ( A_{\Phi_k} \, B_{\Phi_k} \right )
% % 	\end{align*}
% % 	%
% % 	where
% % 	%
% % 	\begin{align*}
% % 		A_{\Phi_k} := U_{\Phi_k,\eps}(\tau,t)\;
% % 		\gamma^{\Phi_k,\eps}_t \left ( J \, \frac{1}{H - \xi} \right ) \;M_{\Phi_k,\eps}(t,\tau) \in \Alg
% % 	\end{align*}
% % 	%
% % 	and
% % 	%
% % 	\begin{align*}
% % 		B_{\Phi_k} := \gamma^{\Phi_k,\eps}_{\tau} \bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr ) \in \mathfrak{L}^1(\Alg)
% % 		.
% % 	\end{align*}
% % 	%
% % 	The sequence $A_{\Phi_k}$ is the product of three equibounded and strongly converging sequences in $\Alg$ when $\Phi_k \to 0$. According to Corollary~\ref{dynamics:cor:Phi_0_limit_perturbed_dynamics} the full propagator $U_{\Phi_k,\eps}(\tau,t) \to U_0(\tau-t)$ converges strongly to the unperturbed one, $\gamma^{\Phi_k,\eps}_t(T) = T$ in view of the strong convergence $G_{\Phi_k,\eps}(t) \to \id$ and $M_{\Phi_k,\eps}(t,\tau) \to U_0(t-\tau)$ in view of Proposition~\ref{dynamics:prop:M_limit_Phi}. As a consequence of the fact that product is continuous in the SOT when the sequences are equibounded one obtains that $A_{\Phi_k}$ is an equibounded sequence such that
% % 	%
% % 	\begin{align*}
% % 		\slim_{\Phi_k \to 0} A_{\Phi_k} = U_0(\tau-t) \, \left ( J \, \frac{1}{H - \xi} \right ) \, U_0(t-\tau)
% % 		.
% % 	\end{align*}
% % 	%
% % 	On the other side
% % 	%
% % 	\begin{align*}
% % 		\norm{\cdot}_1-\lim_{\Phi_k \to 0} B_{\Phi_k} = (H - \xi) \, \partial_{X_j}(\rho)
% % 	\end{align*}
% % 	%
% % 	due to Proposition~\ref{dynamics:prop:interaction_dynamics} (2). In conclusion, the application of Lemma~\ref{framework:lem:strong_convergence_trace_product} and the continuity of the trace with respect to the topology of $\mathfrak{L}^1(\Alg)$ ensure that
% % 	%
% % 	\begin{align*}
% % 		\lim_{\Phi_k \to 0} \mathcal{T} &\left (
% % 		J_{\Phi_k,\eps}(t) \; \alpha^{\Phi_k,\eps}_{(t,\tau)} \bigl ( \partial_{X_j} \bigl ( \rho_{\mathrm{int}}(\tau) \bigl ) \bigr ) \right )
% % 		= \\
% % 		&= \mathcal{T} \left ( U_0(\tau-t) \left ( J \, \frac{1}{H - \xi} \right ) \, U_0(t-\tau) \, (H - \xi) \, \partial_{X_j}(\rho) \right )
% % 		\\
% % 		&= \mathcal{T} \left ( \left ( J \, \frac{1}{H - \xi} \right ) \, (H - \xi) \, U_0(t-\tau) \, \partial_{X_j}(\rho) \, U_0(\tau-t) \right )
% % 		\\
% % 		&= \mathcal{T} \left ( \left ( J \, \frac{1}{H - \xi} \right ) (H - \xi) \; \alpha^0_{t-\tau} \bigl ( \partial_{X_j}(\rho) \bigr ) \right )
% % 		 \\
% % 		&= \mathcal{T} \Bigl ( J \, \alpha^0_{t-\tau} \bigl ( \partial_{X_j}(\rho) \bigr ) \Bigr )
% % 	\end{align*}
% % 	%
% % 	% CHANGED Rename label
% % 	where we used the cyclic property of the trace, the commutativity between $H$ and the unperturbed evolution $\alpha^0_t$ (\cf Corollary~\ref{dynamics:prop:density_core_Liouvillian}) and Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}~(2). This concludes the proof.
% % \end{proof}
% % %
% % Equation~\eqref{main_results:eqn:Kubo_formula} is usually known as the \emph{Kubo formula}.
% % % Is interesting to notice that one can omit condition  in the claim of Theorem~\ref{main_results:thm:Kubo_formula} if one changes Assumption~(IS2) with its stronger version (IS2') (\cf Lemma~\ref{Kubo_formula:lem:Lp_regularity_states} (3)).
% %
% % After a change of variables $\tau \mapsto t - \tau$ in the formula \eqref{main_results:eqn:Kubo_formula}, we obtain
% % %
% % \begin{align}
% % 	\sigma^{\eps}_k[J,\rho](t) = - \ii \, \mathcal{T} \left ( \int^{+\infty}_0 \dd \tau \; \switch(t-\tau) \, f_k(t-\tau) \, J \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr ) \right )
% % 	\label{Kubo_formula:eqn:conductivity_tensor}
% % \end{align}
% % %
% % where the ability to exchange taking the trace and integration is guaranteed by Lemma~\ref{Kubo_formula:lem:existence_integral_net_current}. By using the explicit definition of the {switch on function} $\switch$ one obtains the splitting
% % \eqref{main_results:eqn:Kubo_formula_splitting},
% % %
% % \begin{align*}
% % 	\sigma^{\eps}_k[J,\rho](t) = \widetilde{\sigma}^k_{\eps}[J,\rho](t) + \delta^k_{\eps}[J,\rho](t)
% % 	,
% % \end{align*}
% % %
% % with $\widetilde{\sigma}^k_{\eps}[J,\rho](t)$ given by the formula \eqref{main_results:eqn:Kubo_formula_non_trivial_contribution_splitting}
% % and the remainder
% % %
% % \begin{align}
% % 	\delta^k_{\eps}[J,\rho](t) := \ii \, \mathcal{T} \left ( \int^{t}_0 \dd \tau \; \bigl ( \e^{\eps (t-\tau)} - 1 \bigr ) \, f_k(t-\tau) \,
% % 	J \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr ) \right )
% % 	.
% % 	\label{Kubo_formula:eqn:conductivity_tensor_splitting_remainder}
% % \end{align}
% % %
% % In the adiabatic limit $\eps \to 0^+$ this term plays no role.
% % %
% % \begin{lemma}\label{Kubo_formula:lem:residual_term_vanishes_in_adiabatic_limit}
% % 	Under the hypotheses of Theorem~\ref{main_results:thm:Kubo_formula} it holds that
% % 	%
% % 	\begin{align*}
% % 		\lim_{\eps \to 0^+} \delta^k_{\eps}[J,\rho](t) = 0
% % 		.
% % 	\end{align*}
% % 	%
% % \end{lemma}
% % %
% % %
% % \begin{proof}
% % 	The two inequalities
% % 	%
% % 	\begin{align*}
% % 		\bnorm{\delta^k_{\eps}[J,\rho](t)} &\leqslant \Bigl ( \max_{\tau \in [0,t]} \babs{f_k(t-\tau)} \Bigr ) \; \int^{t}_0 \dd \tau \; \babs{\e^{\eps (t-\tau)} - 1} \;
% % 		\bnorm{J \; \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr )}_1
% % 	\end{align*}
% % 	%
% % 	and
% % 	%
% % 	\begin{align*}
% % 		\Bnorm{J \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr )}_1 &\leqslant \norm{J \, \frac{1}{H - \xi}} \,
% % 		\Bnorm{(H - \xi) \; \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr )}_1\\
% % 		&\leqslant \norm{J \, \frac{1}{H - \xi}} \,
% % 		\Bnorm{(H - \xi) \, \partial_{X_j}(\rho)}_1
% % 		,
% % 	\end{align*}
% % 	%
% % 	Dominated Convergence and the fact $\babs{\e^{\eps (t-\tau)} - 1} \to 0$ when $\eps \to 0^+$ are enough to prove the claim.
% % \end{proof}
% % %
% % %
% % \begin{proof}[Corollary~\ref{main_results:cor:conductivity_tensor_special_cases}]
% % 	%
% % 	\begin{enumerate}
% % 		\item The equality
% % 		%
% % 		\begin{align*}
% % 			J \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(\rho) \bigr ) = \left ( J \, \frac{1}{H - \xi} \right ) \alpha^{0}_{\tau} \bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr )
% % 			,
% % 		\end{align*}
% % 		%
% % 		the resolvent formula \eqref{framework:eqn:resolvent_equation_integral} for the $\R$-flow generated by $-H$ (we use $\mathscr{L}_{-H}^{(1)} = -\mathscr{L}_{H}^{(1)}$) and expressing the resolvent of via~\eqref{main_results:eqn:laplace_transform_resolvent} as the Laplace transform of the evolution group yields
% % 		%
% % 		\begin{align}
% % 			\widetilde{\sigma}^k_{\eps}[J,\rho](t) = - \ii \, \e^{\eps t} \; \mathcal{T} \left ( \left ( J \, \frac{1}{H - \xi} \right ) \; \frac{1}{\mathscr{L}_{H}^{(1)} + \eps} \bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr ) \right )
% % 			.
% % 			\label{Kubo_formula:eqn:conductivity_tensor_before_eps_limit}
% % 		\end{align}
% % 		%
% % 		Under the assumptions of Theorem~\ref{main_results:thm:Kubo_formula} both $(H - \xi) \, \partial_{X_j}(\rho) $ and $\partial_{X_j}(\rho)$ are elements of $\mathfrak{L}^1(\Alg)$. Moreover, $\mathscr{L}_H^{(1)} \bigl ( g(H) \, A \bigr ) = g(H) \, \mathscr{L}_H^{(1)}(A)$ for any bounded function $g$ of $H$ and any $A \in \mathfrak{L}^1(\Alg)$. This implies that
% % 		%
% % 		\begin{align*}
% % 			\frac{1}{H - \xi} \, \frac{1}{\mathscr{L}_{H}^{(1)} + \eps} \bigl ( (H - \xi) \, \partial_{X_j}(\rho) \bigr ) &= \frac{1}{\mathscr{L}_H^{(1)} + \eps} \left ( \frac{1}{H - \xi} \, (H - \xi) \, \partial_{X_j}(\rho) \right )
% % 			\\
% % 			&= \frac{1}{\mathscr{L}_H^{(1)} + \eps} \bigl ( \partial_{X_j}(\rho) \bigr )
% % 		\end{align*}
% % 		%
% % 		as elements of $\mathfrak{L}^1(\Alg)$, where in the second equality we used Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}~(1). Finally, the last equality is justified by the condition $\domain(H) \subseteq \domain(J)$ which ensures that the two quantities inside the trace $\mathcal{T}$ agree on a $\mathcal{T}$-dense domain and so as elements of $\mathfrak{L}^1(\Alg)$.
% % 		\item This is just an application of the Fubini-Tonelli theorem to the arguments used to prove Corollary~\ref{main_results:cor:conductivity_tensor_special_cases}.
% % 	\end{enumerate}
% % 	%
% % \end{proof}
% % %
% % subsection the_kubo_formula_for_the_conductivity_tensor (end)
% section the_kubo_formula (end)


\section{Adiabatic limit of the Kubo formula} % (fold)
\label{Kubo_formula:adiabatic_limit}
%
The adiabatic limit of the conductivity tensor corresponds to the computation of the limit $\eps \to 0$ in the Kubo Formula. In order to prove the existence of this limit we need to assume something more about the observable $J$. In fact we need that there is a $Q_J \in \mathfrak{L}^q(\Alg)$ such that $J = \mathscr{L}_H^{(q)}(Q_J)$ where $\mathscr{L}_H^{(q)}$ is the Liouvillian in the space $\mathfrak{L}^q(\Alg)$. Here $\frac{1}{p} + \frac{1}{q} = 1$.
% 
\begin{proof}[Proof of Theorem~\ref{main_results:thm:adiabatic_limit_Kubo_formula}]
	Due to the assumption $H \, \partial_{X_j}(\rho) \in \mathfrak{L}^p(\Alg)$ we can replace in formula \eqref{main_results:eqn:Kubo_formula_Fourier_transform_f} the Liouvillian $\mathscr{L}_H^{(1)}$ with the Liouvillian $\mathscr{L}_H^{(p)}$. Moreover, the trace $\mathcal{T}$ establishes a duality relation between $\mathfrak{L}^q(\Alg)$ and $\mathfrak{L}^p(\Alg)$ which provides
	%
	\begin{align*}
		\mathcal{T} \left ( J \; \frac{1}{\mathscr{L}_H^{(p)}+\eps}(R) \right ) = \mathcal{T} \left ( \frac{1}{-\mathscr{L}_H^{(q)} + \eps}(J) \; R \right ) 
	\end{align*}
	%
	for all $J \in \mathfrak{L}^q(\Alg)$ and $R \in \mathfrak{L}^p(\Alg)$ (\cf the proof of \cite[Lemma 4.2]{Pagter_Sukochev:commutator_estimates_R_flows:2007}). Using this fact in the formula 
	% CHANGED Label undefined 
	\eqref{main_results:eqn:Kubo_formula_Fourier_transform_f} with $J = \mathscr{L}_H^{(q)}(Q_J)$ and $R = \partial_{X_j}(\rho) $ one obtains
	%
	\begin{align}
		\widetilde{\sigma}^k_{\eps}[J,\rho](t) = \ii \, \e^{\eps t} \;
		\mathcal{T} \left ( \frac{\mathscr{L}_H^{(q)}}{\mathscr{L}_H^{(q)} - \eps}(Q_J) \; \partial_{X_j}(\rho) \right ) 
 		.
		\label{Kubo_formula:eqn:Kubo_formula_pre_projection}
	\end{align}
	%
	% CHANGED Labels undefined 
	The inequality \eqref{framework:eqn:trace_Lp_Lq_estimate} allows to compute the limit $\eps \to 0$ inside the trace and from \eqref{main_results:eqn:limit_L_Lplus_eps_projection} one gets
	%
	\begin{align*}
		\lim_{\eps \to 0^+} \widetilde{\sigma}^k_{\eps}[J,\rho](t) = \ii \;
		\mathcal{T} \Bigl ( \bigl ( \id_{\mathfrak{L}^q(\Alg)} - \mathscr{P}_H^{(q)} \bigr ) (Q_J) \; \partial_{X_j}(\rho) \Bigr ) 
		. 
	\end{align*}
	%
	Then, equation \eqref{main_results:eqn:adiabatic_limit_conductivity_tensor} just follows from Lemma~\ref{Kubo_formula:lem:residual_term_vanishes_in_adiabatic_limit}. Formula \eqref{main_results:eqn:adiabatic_limit_L2_conductivity_tensor} follows from \eqref{main_results:eqn:adiabatic_limit_conductivity_tensor} once one uses the definition of the scalar product on $\mathfrak{L}^2(\Alg)$ given in Remark~\ref{framework:remark:abstract_Hilbert_Schmidt_space}.
\end{proof}
% 
% section adiabatic_limit_of_the_kubo_formula (end)


\section{The Kubo-Str\v{e}da formula} % (fold)
\label{Kubo_formula:adiabatic_limit}
%
The Kubo-Str\v{e}da formula concerns the application of the Kubo formula to the case of an initial equilibrium state given by a projection and the observable given by one of the components of the current operator. 

Just let us make a comment about the requirement (iii) of Theorem~\ref{main_results:thm:Kubo_Streda_formula} for the initial equilibrium state $P = P(H)$. This implies that $H \, P = P \, H = P \, H \, P \in \Alg$ (bounded affiliated operator) and, together with Hypothesis~\ref{hypothesis:state}, it implies that $P , H \, P \in \Alg \cap \rr{W}^{1,1}(\Alg) \cap \rr{W}^{1,2}(\Alg)$.

Let $f_n \in C^{\infty}_{\mathrm{c}}(\R)$ be a family of smooth and compactly supported functions such that $\sabs{f_n(x)} \leqslant 1$ for all $x \in \R$ and $f_n(x) = 1$ for all $x \in [-n,n]$. In this way one has that $f_n(H) \in \Alg$, $\bnorm{f_n(H)} = 1$ and $f_n(H) \to \id$ in the SOT. Moreover, in view of Lemma~\ref{Kubo_formula:lem:Lp_regularity_states} we also have that $J_k \, f_n(H) \in \Alg$ since
%
\begin{align*}
	J_k \, f_n(H) = \left ( J_k \, \frac{1}{H - \xi} \right ) \, \bigl ( (H - \xi) \, f_n(H) \bigr ) 
\end{align*}
%
and $(H - \xi) \, f_n(H) \in \Alg$.
% TODO Rewrite proof for special case $q = 2$. 
%
\begin{proof}[of Theorem~\ref{main_results:thm:Kubo_Streda_formula}]
	Let us start with the quantity
	%
	\begin{align*}
		\Sigma_{k,j}(\tau) :& \negmedspace= \mathcal{T} \Bigl ( J_k \; \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(P) \bigr ) \Bigr ) 
		\\
		&= \lim_{n \to +\infty} \mathcal{T} \Bigl ( \bigl ( J_k \, f_n(H) \bigr ) \; \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(P) \bigr ) \Bigr )
	\end{align*}
	%
	which appears as the integrand in the equation 
	% CHANGED Label no longer defined 
	\eqref{Kubo_formula:eqn:conductivity_tensor}. The second equality is consequence of Lemma~\ref{framework:lem:strong_convergence_trace_product} and of the fact that $H \, \partial_{X_j}(P) \in \mathfrak{L}^1(\Alg)$. Using the cyclicity of the trace one obtains
	%
	\begin{align*}
		\Sigma_{k,j}(\tau) &= \lim_{n \to +\infty} \mathcal{T} \Bigl ( \alpha^{0}_{-\tau} \bigl ( J_k \, f_n(H) \bigr ) \; \partial_{X_j}(P) \Bigr ) 
		\\
		&= \lim_{n \to +\infty} \mathcal{T} \left ( \alpha^{0}_{-\tau} \bigl ( J_k \, f_n(H) \bigr ) \; \Bigl [ \, P \, , \, \bigl [ P \, , \, \partial_{X_j}(P) \bigr ]_{(1)} \Bigr ]_{(1)} \right ) 
		\\
		&= \lim_{n \to +\infty} \mathcal{T} \Bigl ( \big[\alpha^{0}_{-\tau} \bigl ( J_k \, f_n(H) \bigr ) \, , \, P \, \bigr ] \; \bigl [ \, P \, , \, \partial_{X_j}(P) \bigr ]_{(1)} \Bigr ) 
		\\
		&= \lim_{n \to +\infty} \mathcal{T} \left ( \Bigl [ \bigl [ \alpha^{0}_{-\tau} \bigl ( J_k \, f_n(H) \bigr ) \, , \, P \bigr ] \, , \, P \Bigr ] \; \partial_{X_j}(P) \right )
	\end{align*}
	%
	where in the second equality we used Lemma~\ref{framework:lem:double_commutator_identity} and in the last two equalities we used equation \eqref{framework:eqn:trace_product_with_commutator_switch} twice with $p = \infty$. The symbol $[ \, \cdot \, , \, \cdot \, ]$ denotes the commutator in $\Alg$. The equilibrium condition $\alpha^{0}_{\tau}(P) = P$ for all $\tau \in \R$ allows to write
	% 
	\begin{align}
		\Sigma_{k,j}(\tau) &= \lim_{n \to +\infty} \mathcal{T} \left ( 
		\alpha^{0}_{-\tau} \left ( \Bigl [ \, P \, , \, \bigl [ P \, , \, J_k \, f_n(H) \bigr ] \Bigr ] \right ) \, \partial_{X_j}(P) \right ) 
		\notag \\
		&= \lim_{n \to +\infty} \mathcal{T} \left ( 
		\Bigl [ \, P \, , \, \bigl [ P \, , \, J_k \, f_n(H) \bigr ] \Bigr ] \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(P) \bigr ) \right ) 
		. 
		\label{Kubo_formula:eqn:Streda_formula_via_auxiliary_limit}
	\end{align}
	% 
	The next step is to prove the following identity
	%
	\begin{align}
		\bigl [ P \, , \, J_k \, f_n(H) \bigr ] = \bigl [ H \, , \, \partial_{X_k}(P) \bigr ]_{\ddagger}\; f_n(H)
		\label{Kubo_formula:eqn:Streda_formula_commutator_identity}
	\end{align}
	%
	where $[\, \cdot \, , \, \cdot \, ]_{\ddagger}$ is the generalized commutators from Definition~\ref{framework:defn:generalized_commutators}. The equilibrium condition implies that $P$ commutes with $H$ and $(H \, P)^* = H \, P$ in view of the fact that both $H$ and $P$ are selfadjoint. Since the derivations $\partial_{X_k}$ are selfadjoint one concludes from 
	% CHANGED Label no longer defined
	\eqref{main_results:eqn:identity_H_partial_X_rho} that
	%
	\begin{align*}
		\bigl [ H \, , \, \partial_{X_k}(P) \bigr ]_{\ddagger} \; f_n(H) &= - \Bigl ( J_k \, P - (J_k \, P)^* \Bigr ) \; f_n(H)\\
		&= - \bigl ( J_k \, P \, f_n(H) \bigr ) + \bigl ( f_n(H) \, J_k \, P \bigr )^*
		\\
		&= - \bigl ( J_k \, f_n(H) \bigr ) \, P + P \, \bigl ( f_n(H) \, J_k \bigr )^*
		\\
		&= - \bigl ( J_k \, f_n(H) \bigr ) \, P + P \, \bigl ( J_k \, f_n(H) \bigr ) 
	\end{align*}
	%
	which is exactly the relation \eqref{Kubo_formula:eqn:Streda_formula_commutator_identity}. Observe that all the equalities in the previous argument make sense in $\mathfrak{L}^1(\Alg)$ and $\mathfrak{L}^q(\Alg)$!!!!. Moreover, $\bigl [ P \, , \, J_k \, f_n(H) \bigr ]_{(1)} = \bigl [ P \, , \, J_k \, f_n(H) \bigr ]$ in view of the fact $P \in \Alg \cap \mathfrak{L}^1(\Alg)$. Combining \eqref{Kubo_formula:eqn:Streda_formula_via_auxiliary_limit} and \eqref{Kubo_formula:eqn:Streda_formula_commutator_identity} one gets after taking the limit $n \to +\infty$
	%
	\begin{align*}
		\Sigma_{k,j}(\tau) &= \mathcal{T} \left ( \Bigl [ \, P \, , \, \bigl [ H \, , \, \partial_{X_k}(P) \bigr ]_{\ddagger} \Bigr ]_{(q)} \, \alpha^{0}_{\tau} \bigl ( \partial_{X_j}(P) \bigr ) \right ) 
		 .
		 % \label{Kubo_formula:eqn:Streda_formula}
	\end{align*}
	%
	Observe that in view of Lemma~\ref{framework:lem:extension_algebra_unbounded_operators}~(1) one has $\bigl ( H \, \partial_{X_k}(P) \bigr ) \, P = H \, \bigl ( \partial_{X_k}(P) \, P \bigr )$. Now we need also $P \, H = H \, P \in \Alg$. Then one has that
	%
	\begin{align*}
		P \, \bigl ( H \, \partial_{X_k}(P) \bigr ) = (PH) \, \partial_{X_k}(P) 
		= H \, \bigl ( P \, \partial_{X_k}(P) \bigr )
	\end{align*}
	%
	which implies
	%
	\begin{align*}
		\Bigl [ P \, , \, \bigl ( H \, \partial_{X_k}(P) \bigr ) \Bigr ]_{(q)} = P \, \bigl ( H \, \partial_{X_k}(P) \bigr ) - \bigl ( H \, \partial_{X_k}(P) \bigr ) \, P 
		= H \, \bigl [ P \, , \, \partial_{X_k}(P) \bigr ]_{(p)}
	\end{align*}
	%
	with the equality which makes sense in $\mathfrak{L}^q(\Alg)$????. Taking the adjoint one gets
	%
	\begin{align*}
		\Bigl [ \, P \, , \, \bigl [ H \, , \, \partial_{X_j}(P) \bigr ]_{\ddagger} \Bigr ]_{(q)} = \Bigl [ \, H \, , \, \bigl [ P \, , \, \partial_{X_j}(P) \bigr ]_{(p)} \Bigr ]_{\ddagger}
	\end{align*}
	%
	This implies that $\bigl [ P \, , \, \partial_{X_j}(P) \bigr ]_{(p)}$ is in the domain of $\mathscr{L}_H^{(q)}$ and
	%
	\begin{align*}
		\Bigl [ \, P \, , \, \bigl [ H \, , \, \partial_{X_k}(P) \bigr ]_{\ddagger} \Bigr ]_{(q)} = \mathscr{L}_H^{(q)} \Bigl ( \bigl [ P \, , \, \partial_{X_k}(P) \bigr ]_{(p)} \Bigr ) 
	\end{align*}
	%
	This implies that we are in the condition to apply Theorem~\ref{main_results:thm:adiabatic_limit_Kubo_formula} which provides
	%
	\begin{align*}
		\sigma_{kj}[P] := \sigma^j[J_k,P] = \ii \Bdscpro{\mathscr{P}_H^{(2)\perp} \bigl [ P \, , \, \partial_{X_k}(P) \bigr ]_{(2)} \; }{ \, \partial_{X_j}(P)}_{\mathfrak{L}^2}
		% \label{Kubo_formula:eqn:Streda_formula}
	\end{align*}
	%
	To conclude the proof we need to show that $\bigl [ P \, , \, \partial_{X_k}(P) \bigr ]_{(2)} \in \ker \bigl (\mathscr{L}_H^{(2)} \bigr )^{\perp}$. Let us start by observing that 
	%
	\begin{align*}
		A \in \ker \bigl ( \mathscr{L}_H^{(2)} \bigr ) 
		\; \; \Longrightarrow \; \; \bigl [ A \, , \, f(H) \bigr ]_{(2)} = 0
		\; \; \Longrightarrow \; \; [A,P]_{(2)} = 0
	\end{align*}
	%
	where $f \in ????$ and $P = f(H)$. Thus
	%
	\begin{align*}
		\Bdscpro{A}{\bigl [ P \, , \, \partial_{X_k}(P) \bigr ]_{(2)}}_{\mathfrak{L}^2} = \Bdscpro{[A,P]_{(2)} \;}{\, \partial_{X_k}(P)}_{\mathfrak{L}^2} 
		= 0
	\end{align*}
	%
	where in the first equality we used the formula \ref{framework:eqn:trace_product_with_commutator_switch}. This provides
	%
	\begin{align*}
		\sigma_{kj}[P] &= \ii \Bdscpro{\bigl [P \, , \, \partial_{X_k}(P) \bigr ]_{(2)}^* \;}{\, \partial_{X_j}(P) }_{\mathfrak{L}^2} 
		\notag \\
		&= - \ii \Bdscpro{\bigl [ \, P \, , \, \partial_{X_k}(P) \bigr ]_{(2)} \;}{\, \partial_{X_j}(P) }_{\mathfrak{L}^2}
		\notag \\
		&= - \ii \Bdscpro{P \,}{\, \bigl [ \partial_{X_k}(P) \, , \, \partial_{X_j}(P) \bigr ]_{(2)}}_{\mathfrak{L}^2}
		% \label{Kubo_formula:eqn:Streda_formula}
	\end{align*}
	%
\end{proof}
% 
% section the_kubo_str_v_e_da_formula (end)
% chapter proofs_chapter_6 (end)


\chapter{Old version of Applications} % (fold)
\label{cha:old_version_of_applications}
%
\section{A generalized framework for physical applications}






%--------%
\section{Some relevant physical application}


%--------%
\subsection{Continuous case vs. discrete }
The two cases of main interest for physical applications
concern $\mathbb{G}=\R^d$ (\emph{continuous case}) and $\mathbb{G}=\Z^d$ (\emph{discrete} or \emph{tight-binding case}). The {configuration} unweighted Hilbert space for the continuous case is
$$
\Hil_{*}:=L^2(\n{R}^d, \dd x)\otimes \C^N
$$
where we used $\dd x$ for the Lebesgue measure. In the discrete case the measure structure on $\Z^d$ is given by the counting (or Dirac) measure $\delta_x$ and consequently one has
$$
\Hil_{*}:=\ell^2(\n{Z}^d)\otimes \C^N
$$

The twisting group 2-cocycle is usually chosen of the form
$$
\Theta(x,y):=\e^{\ii x^t\Theta y}=\e^{\ii\sum_{r,s=1}^d\Theta^{rs}x_r y_s}
$$
where $\Theta^{rs}\in\R$ are the component of an antisymmetric tensor of order two and $x:=(x_1,\ldots,x_d)$, $y:=(y_1,\ldots,y_d)$ are vectors in $\R^d$ or in $\Z^d$. The tensor $\Theta^{rs}$ has usually the meaning of a constant magnetic field. Whit this choice of  twisting group 2-cocycle
the \emph{magnetic translations} $\hat{U}_y$, act as
$$
(\hat{U}_y\hat{\varphi})_{\tau_{y}(\omega)}(x):=(S_y\varphi_{\omega})(x)=\Theta(y,x)\varphi_{\omega}(x-y)\, ,\qquad\quad \hat{\varphi}=\{\varphi_{\omega}\}\in\mathfrak{H}
$$
where $x$ and $y$ are points in $\R^d$ or in $\Z^d$ and we used an additive notation for the group structures.

The typical  generatos for the derivations are the \emph{position operators} $X_j$ defined by
$$
(\hat{X}_j\hat{\varphi})_{\omega}(x):=x_j\varphi_{\omega}(x)\qquad\quad j=1,\ldots,d,\ \ \omega\in\Omega.
$$
where $x_j$ is the $j$-th components of the vector $x$.

The main difference between the continuous and the discrete case concerns the trace por
trace per unit volume. In the continuous case one has the typical representations
$$
\begin{aligned}
\bb{T}_{\n{P}}(\hat{A})&= \int_{\Omega}{\rm Tr}_{\Hil_{\omega}}(P_{\Lambda_0}A_{\omega} P_{\Lambda_0}) \ \dd\n{P}(\omega)\\
&=\lim_{n\to\infty}\frac{1}{(2n+1)^d}\int_{\Omega}{\rm Tr}_{\Hil_{\omega}}
(P_{\Lambda_n}A_{\omega} P_{\Lambda_n})\  \dd\n{P}(\omega).
\end{aligned}
$$
where $P_{\Lambda_n}$ is the multiplication operator for the characteristic function of the cube $\Lambda_n:=[-n-1/2,+n+1/2]^d$ (in fact, a projection). Clearly this trace is only semi-finite and not finite since $\bb{T}_{\n{P}}(\hat{\id})=+\infty$. In the discrete case one has
$$
\begin{aligned}
\bb{T}_{\n{P}}(\hat{A})&= \int_{\Omega}{\rm Tr}_{\Hil_{\omega}}({\delta_0}A_{\omega} {\delta_0}) \ \dd\n{P}(\omega)\\
&=\lim_{n\to\infty}\frac{1}{(2n+1)^d}\int_{\Omega}{\rm Tr}_{\Hil_{\omega}}
(P_{\Lambda_n}A_{\omega} P_{\Lambda_n})\  \dd\n{P}(\omega).
\end{aligned}
$$
where $\delta_j$ is the projection on the site $j$-th of the lattice $\Z^d$ and 
$P_{\Lambda_n}:=\sum_{j\in\Lambda_n\cap\Z^d} \delta_j$. In this case a simple computation shows that  
$$
\bb{T}_{\n{P}}(\hat{\id})=\int_{\Omega}{\rm Tr}_{\C^N}(W_{\omega}(0))\ \dd\n{P}(\omega)<+\infty
$$
namely the trace turns out to be finite. For this reason all the simplifications sketched in Section \ref{main_results:tight_binding_simplification} apply. 




%--------%
\subsection{Quantum Hall Effect}
The derivation of the Hall conductivity for the Quantum Hall Effect
is the real case study for the LRT. For this case the spinorial degrees of freedom are not relevant, hence $N=1$. Also the field of weights plays no role in such a way that one can set $W\equiv1$.


Let us start from the discrete case. In absence of disorder the first mathematically rigorous work dates back to D. J. Thouless et al. \cite{Thouless_Kohmoto_Nightingale_Den_Nijs:quantized_hall_conductance:1982}. The Hamiltonian  is described by the \emph{Hofstadter model}
$$
H_B:=T_{B,1}+T_{B,1}^*+T_{B,2}+T_{B,2}^*
$$
defined on the Hilbert space $\Hil:=\ell^2(\Z^2)$ by means of the generators
$$
(T_{B,1}\varphi)(n_1,n_2):=\e^{+ \ii\Theta_Bn_2}\varphi(n_1-1,n_2),\qquad (T_{B,2}\varphi)(n_1,n_2):=\e^{- \ii\Theta_Bn_1}\varphi(n_1,n_2-1)
$$
where $n=(n_1,n_2)\in\Z^2$ and $\varphi\in \ell^2(\Z^2)$. The quantity $\Theta_B\in\R$ represents the flux for unit cell of a uniform magnetic field $B$. The generators $T_{B,1}$ and $T_{B,2}$, and therefore the Hamiltonian $H_B$, commute with respect to the 
\emph{magnetic translations}
$$
(S_{B,1}\varphi)(n_1,n_2):=\e^{+ \ii\Theta_Bn_2}\varphi(n_1+1,n_2),\qquad (S_{B,2}\varphi)(n_1,n_2):=\e^{+ \ii\Theta_Bn_1}\varphi(n_1,n_2-1).
$$
A direct computation shows that $[T_{B,j},S_{B,k}]=0$ for $j,k=1,2$ and this means that
the Hamiltonian $H_B$ is an element of the von Neumann algebra
$$
\Alg_{\n{Z}^2}:={\rm Span}_\n{\n{Z}^2}\{S_{B,1},S_{B,2}\}'\cap\mathscr{B}(\ell^2(\Z^2)).
$$ 
In fact the magnetic translations $S_{B,1}$ and $S_{B,2}$ are the generator of a projective representation of the group $\n{Z}^2$ given by $(1,0)\mapsto S_{B,1}$ and 
$(0,1)\mapsto S_{B,2}$ and commutation relations
$$
S_{B,1}S_{B,2}=\e^{+ \ii2\Theta_B}\,S_{B,2}S_{B,1}
$$
which are compatible with the twisting cocycle $\Theta(n,m):=\e^{\ii\Theta_B(n_1m_2-n_2m_1)}$ for all $n=(n_1,n_2)$ and $m=(m_1,m_2)$ in $\Z_2$. The LRT is obtained by choosing $J_1:=\ii[H_B, X_1]$ as observable, $G_{\Phi,\eps}(t) := \e^{+ \ii \int_{-\infty}^t\dd\tau s_\eps(\tau)\Phi X_2}$, with $\eps>0$ and $\Phi\in\R$ as perturbation and $P_E:=\chi_{(-\infty,E]}(H_B)$ as initial equilibrium state with $E$ in a spectral gap of $H_B$. Since all the Hypothesis for the validity of the LRT hold (even in the simplified form of Section \ref{main_results:tight_binding_simplification}) one immediately deduces the  Kubo-Str\v{e}da formula \eqref{main_results:eqn:Kubo_Streda_formula} which is explicitly given by
%
\begin{equation}\label{eq:QHE-01}
\sigma^{12}[P_E]:=\ii
{\rm Tr}_{\ell^2(\Z^2)}\Big({\delta_0}\,
P_E\,\big[[X_1,P_E],[X_2,P_E]\big]_{(1)}{\delta_0}\Big).
\end{equation}
%
The same formula holds whenever the  Hofstadter model $H_B$ is replaced by any element in the von Neumann algebra $\Alg_{\n{Z}^2}$ provided that $P_E$ is still a spectral projection into a gap. In fact this condition, which is equivalent to a fast decay of the matrix elements of $P_E$ assure that $\big[[X_1,P_E],[X_2,P_E]\big]_{(1)}$ is in the right class with respect to the trace per unit volume (\ie the Sobolev condition $P_E\in \rr{W}^{1,1}(\Alg_{\n{Z}^2}) \cap \rr{W}^{1,2}(\Alg_{\n{Z}^2})$). 
When $\Theta_B=\pi\n{Q}$ (rational flux condition) it is possible to find an abelian subalgebra of  ${\rm Span}_\n{\n{Z}^2}\{S_{B,1},S_{B,2}\}$ and one can use the Gel'fand-Fourier (Bloch-Floquet) transform in order to recover from 
\eqref{eq:QHE-01} the celebrated (commutative) Kubo-Chern formula \cite[eq. (5)]{Thouless_Kohmoto_Nightingale_Den_Nijs:quantized_hall_conductance:1982}.

\medskip

The discrete case with disorder has been extensively studied in \cite{Bellissard_van_Elst_Schulz_Baldes:noncommutative_geometry_quantum_Hall_effect:1994,Bellissard_Schulz_Baldes:quantum_transport_aperiodic_media:1998}. The only differences with respect to the non-random case are that now the Hilbert space is given by the direct integral
$$
\mathfrak{H}:=\int^\oplus_\Omega\ell^2(\Z^2)\ \dd\n{P}(\omega)\simeq L^2(\Omega,\n{P})\otimes \ell^2(\Z^2)
$$ 
and that the Hamiltonian $H_B:=\{H_{B,\omega}\}$ is a covariant element with respect to the magnetic translations, \ie an element of
$$
\Alg(\Omega,\n{Z}^2,\n{P}):={\rm Span}_{\Z^2}\{\hat{U}_{B,1},\hat{U}_{B,2}\}'\cap\mathrm{Rand}(\widehat{\Hil})
.
$$
In this case the the formula for the conductivity results
%
\begin{equation}\label{eq:QHE-02}
\sigma^{12}[P_E]:=\ii\int_{\Omega}
{\rm Tr}_{\ell^2(\Z^2)}\Big({\delta_0}\,
P_{E,\omega}\,\big[[X_1,P_{E,\omega}],[X_2,P_{E,\omega}]\big]_{(1)}{\delta_0}\Big)\ \dd\n{P}(\omega)
\end{equation}
%
where the spectral projection $P_E=\{P_{E,\omega}\}$ is subjected to the condition of lying in a zone of dynamical localization which is equivalent to the  the Sobolev condition $P_E\in \rr{W}^{1,1}(\Alg(\Omega,\n{Z}^2,\n{P})) \cap \rr{W}^{1,2}(\Alg(\Omega,\n{Z}^2,\n{P}))$. 


The continuous case has been treated rigorously in \cite{Elgart_Schlein:Kubo_for_Landau:2004} in absence of disorder and in \cite{Bouclet_Germinet_Klein_Schenker:linear_response_theory_magnetic_Schroedinger_operators_disorder:2005,klein-lenoble-muller-07,Dombrowski_Germinet:linear_response_theory_non_commutative_integration:2008} in the case with disorder. In absence of disorder the basic model is described by the \emph{Landau Hamiltonian}
%
\begin{equation}\label{eq:QHE-03}
H({\bf A},V):=(- \ii\nabla+{\bf A})^2+V
\end{equation}
%
acting on the Hilbert space $L^2(\R^2,\dd x)$. The \emph{magnetic} potential ${\bf A}$ and the electric potential $V$ have to meet the Leinfelder-Simader conditions in such a way that  $H({\bf A},V)$ is essentially selfadjoint on $C_{\rm c}^{\infty}(\R^2)$ \cite[Theorem 3]{Leinfelder1981}. The magnetic part $(- \ii\nabla+{\bf A})^2$ is invariant under the representation of the magnetic translations $\R^2\ni x\mapsto S_{B,x}$ described in \cite{Arai1992}. The random model is obtained by promoting the two potentials to covariant random variables, \ie to maps $\Omega\ni\omega\mapsto {\bf A}_{\omega}$ and $\Omega\ni\omega\mapsto V_{\omega}$ such that ${\bf A}_{\omega}$ and $V_{\omega}$ verify the Leinfelder-Simader conditions for $\n{P}$-almost all $\omega$ and the operator valued map  $\Omega\ni\omega\mapsto H_{\omega}:=H({\bf A}_{\omega},V_{\omega})$ is measurable and covariant in the sense that
$$
U_{B,x,\tau_{x}(\omega)}\,H_{\omega}\,U_{B,x,\tau_{x}(\omega)}^* = H_{\tau_{x}(\omega)}\qquad\quad x\in\n{R}^2,\ \ \omega\in\Omega.
$$
%
Here the operators $\hat{U}_{B,x}$ provides the extension of the magnetic translations
$S_{B,x}$ to the direct integral
$$
\mathfrak{H}:=\int^\oplus_\Omega L^2(\R^2,\dd x)\ \dd\n{P}(\omega)\simeq L^2(\Omega,\n{P})\otimes L^2(\R^2,\dd x)
$$ 
according to the usual prescription. This assures that $H:=\{H_{\omega}\}$ is an element affiliated with the von Neumann algebra
$$
\Alg(\Omega,\n{R}^2,\n{P}):={\rm Span}_{\n{R}^2}\{\hat{U}_{B,x}\}'\cap\mathrm{Rand}(\widehat{\Hil})
.
$$ 
Assuming as initial equilibrium state a spectral projection $P_E=\{P_{E,\omega}\}$ of $H$
 subjected to the condition of lying in a zone of dynamical localization (\ie  the Sobolev condition $P_E\in \rr{W}^{1,1}(\Alg(\Omega,\n{Z}^2,\n{P})) \cap \rr{W}^{1,2}(\Alg(\Omega,\n{Z}^2,\n{P}))$) one obtains the  Kubo-Str\v{e}da formula
%
\begin{equation}\label{eq:QHE-04}
\sigma^{12}[P_E]:=\ii\int_{\Omega}
{\rm Tr}_{L^2(\R^2,\dd x)}\Big({P_{\Lambda_0}}\,
P_{E,\omega}\,\big[[X_1,P_{E,\omega}],[X_2,P_{E,\omega}]\big]_{(1)}{{P_{\Lambda_0}}}\Big)\ \dd\n{P}(\omega)
\end{equation}
%

%--------%
\subsection{Maxwell operartor}

In order to describe the \emph{random Maxwell operator} we need to work on the reference 
$$
\Hil_{*}:=L^2(\n{R}^3, \dd x)\otimes \C^6
$$
and we need a field of weights $\Omega\ni\omega\mapsto W_{\omega}\in L^{\infty}(\n{R}^3,\dd x)\otimes{\rm Mat}(\C^6)$ which meets the conditions of Definition \ref{def:field_weights}. The {Maxwell operator} $M:=\{M_{\omega}\}$ is the collection of operator defined by
$$
M_{\omega}:=W_{\omega}^{-1} M_0
$$
where the operator
$$
M_0:=\left(\begin{array}{c|c}
0 & - \ii\nabla^\times \\
\hline
+ \ii\nabla^\times & 0\end{array}\right)
$$
contains in the off-diagonal part the curl operator $\nabla^\times$. It is well known that $M_{\omega}$ is selfadjoint on the 
{weighted} 
  Hilbert spaces
$$
\Hil_{\omega}:=[L^2(\n{R}^3, \dd x)\otimes \C^6]_{W_{\omega}}
$$
with domain $H^1(\n{R}^3, \dd x)\otimes \C^6$ (here we use the simplification of not considering the constraints on the domain that assure the absence of sources). Let consider on the direct integral
$$
\mathfrak{H}:=\int^\oplus_\Omega [L^2(\n{R}^3, \dd x)\otimes \C^6]_{W_{\omega}}
\ \dd\n{P}(\omega)
$$ 
the unitary representation $\R^3\ni a\mapsto \hat{U}_{a}$ given by 
$$
(\hat{U}_x\hat{\varphi})_{\tau_{a}(\omega)}(x):=\varphi_{\omega}(x-a)\, ,\qquad\quad \hat{\varphi}=\{\varphi_{\omega}\}\in\mathfrak{H}
$$
(in this case the twisting cocycle is just $\Theta=0$).
As a consequence of Proposition \ref{propos:affiliation} it follows that $M$ is affiliated with the von Neumann algebra
$$
\Alg(\Omega,\n{R}^3,\n{P}):={\rm Span}_\mathbb{G}\{\hat{U}_x\}'\cap\mathrm{Rand}(\widehat{\Hil})
.
$$ 
This algebra is endowed with the trace per unit volume $\bb{T}_{\n{P}}$ and a set of compatible generators is given by the position operators $X_1$, $X_2$ and $X_3$. If one set as observable the density of current $J_1:=\{J_{1,\omega}\}$ with $J_{1,\omega}:=\ii[M_{\omega}, X_1]$ and as a (non random) perturbation  
$\hat{G}_{\Phi,\eps}(t) := \{{G}_{\Phi,\eps,\omega}(t)={G}_{\Phi,\eps}(t)\}$ with 
${G}_{\Phi,\eps}(t):=\e^{+ \ii \int_{-\infty}^t\dd\tau s_\eps(\tau)(\Phi_2 X_2+\Phi_3 X_3)}$ one can check (quite easily) that all the Hypothesis are satisfied. Then, if $P_\nu:=\{P_{\nu,\omega}\}$ is a spectral projection of $M$ in a spectral gap or in a spectral region where the Sobolev condition is verified (this part has to be verified in a future work) one can obtain the 
Kubo-Str\v{e}da formula
%
\begin{equation}\label{eq:QHE-06}
\sigma^{1j}[P_E]:=\ii\int_{\Omega}
{\rm Tr}_{\Hil_{\omega}}\Big({P_{\Lambda_0}}\,
P_{\nu,\omega}\,\big[[X_1,P_{\nu,\omega}],[X_j,P_{\nu,\omega}]\big]_{(1)}{{P_{\Lambda_0}}}\Big)\ \dd\n{P}(\omega)
\end{equation}
%
with $j=1,2$. This quantity is related with the transport of energy due to the Poynting vector ${\bf S}$ due to its  relation with the expectation values of the quantity $J_{k,\omega}:=\ii[M_{\omega}, X_k]$ (REF our work). We will explore this facts in a future work.







% chapter old_version_of_applications (end)

==> part.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% {framework:remark:comparison_two_commutators}ample part title
%
% U{framework:remark:comparison_two_commutators}e thi{framework:remark:comparison_two_commutators} file a{framework:remark:comparison_two_commutators} a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% {framework:remark:comparison_two_commutators}pringer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent U{framework:remark:comparison_two_commutators}e the template \emph{part.tex} together with the {framework:remark:comparison_two_commutators}pringer document cla{framework:remark:comparison_two_commutators}{framework:remark:comparison_two_commutators} {framework:remark:comparison_two_commutators}VMono (monograph-type book{framework:remark:comparison_two_commutators}) or {framework:remark:comparison_two_commutators}VMult (edited book{framework:remark:comparison_two_commutators}) to {framework:remark:comparison_two_commutators}tyle your part title page and, if de{framework:remark:comparison_two_commutators}ired, a {framework:remark:comparison_two_commutators}hort introductory text (maximum one page) on it{framework:remark:comparison_two_commutators} ver{framework:remark:comparison_two_commutators}o page in the {framework:remark:comparison_two_commutators}pringer layout.

\end{partbacktext}

==> preface.tex <==
\preface

